Everything is an Operational View: UI as a Projection over Context in Agentic Systems

The emergence of generative AI has enabled Generative User Interfaces (GenUI) that dynamically construct interfaces from user intent, yet existing approaches rely on request-response pipelines that fragment context and limit transparency and control. This paper proposes AFS-UI, which reconceptualises UI as projections over context built on an agentic file-system abstraction that organizes data, capabilities, and interaction state within a unified, persistent workspace. In particular, AFS-UI addresses key limitations in current systems, including heterogeneous resource discoverability, incompatible operation semantics, tangling projection and context, rigid source composition and substitution, and limited evolvability. Within this framework, interfaces become dynamic, inspectable views over shared resources, supporting both human and agent interaction through a common operational surface.

==> tables/existingSystemProtocolsComparison.tex <==
\begin{table*}[t]
\caption{Comparison of generative UI systems and protocols. \zc{Do not feel we need this table. Those protocols map to AUP, not really comparable to AFS-UI as a whole. Maybe just briefly explain these protocol and say AUP is inspired by A2UI and explain what role it plays inside AFS-UI.} %AG-UI focuses on communication, A2UI and Open/JSON-UI on declarative UI generation, and MCP-UI on tool-scoped UI embedding. AFS-UI differs by treating UI as a persistent, agent-readable file-system abstraction, unifying interaction, state, and long-lived context.
}
\centering
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{p{2.2cm} p{2.5cm} p{3cm} p{3.5cm} p{3.5cm} p{3.5cm}}
\toprule
\textbf{System} &
\textbf{Primary \newline Abstraction} &
\textbf{Architectural Role} &
\textbf{Interaction Model} &
\textbf{Rendering Strategy} &
\textbf{State \& Persistence \newline Semantics} \\
\midrule

\textbf{AG-UI} &
Event stream &
Agent--UI communication protocol &
Bidirectional, event-driven message and state synchronization &
No UI rendering; events consumed by frontend frameworks &
Transient session state; persistence handled externally \\

\textbf{A2UI} &
Declarative UI \newline schema &
Agent-generated UI description layer &
Agent emits structured UI components and intents &
Client-side rendering via predefined widget catalogs &
No intrinsic persistence model; UI state managed by host application \\

\textbf{Open-JSON-UI} &
Declarative JSON schema &
Model-agnostic generative UI specification &
Agent outputs JSON-encoded UI structures &
Client interprets schema to construct interactive UI &
Stateless by design; persistence out of scope \\

\textbf{MCP-UI} &
UI resource \newline extension &
Tool-level UI integration over MCP &
UI returned as part of tool execution lifecycle &
Isolated rendering via iframe or remote DOM &
Ephemeral, tool-scoped state; limited persistence \\

\midrule
\textbf{AFS-UI} &
\textbf{File-system view} &
\textbf{Integrated agentic UI framework} &
\textbf{File- and state-driven agent--UI interaction} &
\textbf{UI derived from structured, agent-readable file-system state} &
\textbf{Persistent, versioned state unified with agent actions} \\
\bottomrule
\end{tabular}
}
\end{table*}
